Budget-Constrained Multi-Armed Bandits with Multiple Plays

We study the multi-armed bandit problem with multiple plays and a budget constraint for both the stochastic and the adversarial setting. At each round, exactly $K$ out of $N$ possible arms have to be played (with $1\leq K \leq N$). In addition to observing the individual rewards for each arm played, the player also learns a vector of costs which has to be covered with an a-priori defined budget $B$. The game ends when the sum of current costs associated with the played arms exceeds the remaining budget. Firstly, we analyze this setting for the stochastic case, for which we assume each arm to have an underlying cost and reward distribution with support $[c_{\min}, 1]$ and $[0, 1]$, respectively. We derive an Upper Confidence Bound (UCB) algorithm which achieves $O(NK^4 \log B)$ regret. Secondly, for the adversarial case in which the entire sequence of rewards and costs is fixed in advance, we derive an upper bound on the regret of order $O(\sqrt{NB\log(N/K)})$ utilizing an extension of the well-known $\texttt{Exp3}$ algorithm. We also provide upper bounds that hold with high probability and a lower bound of order $\Omega((1 - K/N)^2 \sqrt{NB/K})$.

==> Sections/AdversarialCase.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% This is AdversarialCase.tex (part of BudgetConstrainedMAB.tex)
% author: Datong Zhou
% last edited: August 17, 2017
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% !TEX root = ../BudgetConstrainedMAB.tex
\section{Adversarial Case}
We now consider the adversarial case, which was first analyzed by \cite{Auer:2002aa} for the single play case (i.e. $K = 1$) and an oblivious adversary. That is, the entire seqence of rewards for all arms is fixed in advance and in particular cannot be adaptively changed during runtime. The proposed algorithm \texttt{Exp3} achieves a regret of $O(\sqrt{NT\log N})$, where $N$ is the number of arms and $T$ the number of rounds to be played. The setting with multiple plays under \textit{bandit} feedback, where only the sum of rewards / losses is observed, was analyzed in \cite{Cesa-Bianchi:2009aa} {\textcolor{red}{Explain a bit more}}. Under \textit{semi-bandit} feedback, where the rewards are observed for each arm pulled, \cite{Uchiya:2010aa} derived a variation of the single-play \texttt{Exp3} algorithm, which they called \texttt{Exp3.M} and enjoys regret $O\left(\sqrt{KTN\log(N/K)} \right)$, where $K$ is the number of plays per round.

We now consider a similar setting with $N$ arms. At each round, the player has to pull exactly $1\leq K \leq N$ arms, as in the setting of \cite{Uchiya:2010aa}. For each arm $i$ pulled at round $t$, the player observes the reward $r_i(t)\in [0, 1]$, but in addition also the cost $c_i(t)\in [c_{\min},1]$, with $0 < c_{\min} < 1$. Further, the player has a budget $B > 0$ to pay for the costs incurred. The algorithm terminates after $\tau_{\mathcal{A}}(B)$ rounds when the sum of materialized costs exceeds the remaining budget. The gain of algorithm $\mathcal{A}$ is the sum of observed rewards up to and including round $\tau_{\mathcal{A}}(B) - 1$.

\subsection{Algorithm \texttt{Exp3.M.B}}
Algorithm \ref{alg:Adversarial_Budget_Constrained} provides the pseudo-code of the budget constrained, multi-armed bandit algorithm under multiple play against an oblivious adversary. Similar to the original \texttt{Exp3} algorithm developed by \cite{Auer:2002aa}, Algorithm \texttt{Exp3.M.B} maintains a set of time-varying weights $\lbrace w_i(t)\rbrace_{i=1}^N$ for all arms, from which the probabilities for each arm being pulled at time $t$ are calculated (line \ref{alg:calculate_probabilities_adversarial}). As noted in \cite{Uchiya:2010aa}, the probabilities $\lbrace p_i(t)\rbrace_{i=1}^N$ sum to $K$ (because exactly $K$ arms need to be pulled), which requires the weights to be capped at a value $v_t > 0$ (line \ref{alg:v_calculation_adversarial}) such that the probabilities $\lbrace p_i(t)\rbrace_{i=1}^N$ are kept in the range $[0, 1]$. At each round, the player draws a set of distinct arms $S(t)$ of cardinality $|S(t)|=K$, where each arm has probability $p_i(t)$ of being included in $S(t)$ (line \ref{alg:dependent_rounding}). This is done by employing algorithm \texttt{DependentRounding} introduced by \cite{Gandhi:2006aa}, which runs in $O(K)$ time and space. At the end of each round, the observed rewards and costs for the pulled arms are turned into estimates $\hat{r}_i(t)$ and $\hat{c}_i(t)$ such that $\mathbb{E}[\hat{r}_i(t)~|~S(t), \ldots, S(1)] = r_i(t)$ and $\mathbb{E}[\hat{c}_i(t)~|~S(t), \ldots, S(1)] = c_i(t)$ for $i\in S(t)$ (line \ref{alg:update_weights_adversarial}). Arms with $w_i(t) < v_t$ are updated according to $(\hat{r}_i(t) - \hat{c}_i(t))$, which assigns larger weights as $\hat{r}_i(t)$ increases and $\hat{c}_i(t)$ decreases.

\begin{algorithm}[h!]
\caption{\texttt{Exp3.M.B}: Budget Constrained Multi-Armed Bandit, Multiple Play, Adversarial}
\label{alg:Adversarial_Budget_Constrained}
\textbf{Input:} Budget $B > 0$, arms $1, \ldots, N$, $K$, parameter $\gamma \in (0,1]$. \\
\textbf{Initialize:} $w_i = 1$ for $i\in [N]$
\begin{algorithmic}[1]
\WHILE {$B > 0$}
\IF {$\arg\max_{i\in [N]} w_i(t) \geq \left(\frac{1}{K} - \frac{\gamma}{N} \right)\sum_{j=1}^N \frac{w_i(t)}{1-\gamma}$}
\STATE Determine $v_t$ as follows:
\begin{align*}
\frac{v_t}{\sum_{i=1}^N v_t \cdot\mathds{1}(w_i(t) \geq v_t) + w_i(t)\cdot\mathds{1}(w_i(t) < v_t)} = \frac{1/K - \gamma/N}{1-\gamma}
\end{align*}\label{alg:v_calculation_adversarial}
\STATE Define set $\tilde{S}(t) = \lbrace i\in [N]~|~w_i(t) \geq v_t\rbrace$.
\STATE Define weights $\tilde{w}_i(t) = v_t$ for $i\in\tilde{S}(t)$.
\ELSE
\STATE Define set $\tilde{S}(t) = \lbrace\rbrace$.
\ENDIF{}
\STATE Define weights $\tilde{w}_i(t) = w_i(t)$ for $i\in [N]\setminus \tilde{S}(t)$.
\STATE Calculate probabilities:
\begin{align*}
p_i(t) = K\left( (1-\gamma)\frac{\tilde{w}_i(t)}{\sum_{j=1}^N \tilde{w}_j(t)} + \frac{\gamma}{N} \right)~\text{for } i\in\tilde{S}(t).
\end{align*}\label{alg:calculate_probabilities_adversarial}
\STATE Draw $S(t) \leftarrow$ \texttt{DependentRounding}$(K, (p_1, \ldots, p_N))$.\label{alg:dependent_rounding}
\STATE Pull arms $S(t)$, observe rewards $r_i(t)\in [0, 1]$ and $c_i(t)\in [c_{\min}, 1]$ for $i\in S(t)$.
\IF {$\sum_{i\in S(t)} c_i(t) > B$}
\RETURN Gain $G_{\texttt{Exp3.M.B}}$, stopping time $\tau_{\mathcal{A}}(B) = t$ \label{alg:return_adversarial}
\ENDIF{}
\STATE $B\leftarrow B - \sum_{i\in S(t)} c_i(t)$.
\STATE $U_{\mathcal{A}} \leftarrow U_{\mathcal{A}} + \sum_{i\in S(t)} r_i(t)$.
\STATE Calculate estimated rewards/costs and update weights for each $i\in [N]$:
\begin{align*}
\hat{r}_i(t) &=
    \begin{cases*}
      r_i(t) / p_i(t) & if $i\in S(t)$ \\
      0        & otherwise
    \end{cases*} \\    
\hat{c}_i(t) &=
    \begin{cases*}
      c_i(t) / p_i(t) & if $i\in S(t)$ \\
      0        & otherwise
    \end{cases*} \\
    w_i(t+1) &=
    \begin{cases*}
      w_i(t) \exp\left( \frac{K\gamma}{N}(\hat{r}_i(t) - \hat{c}_i(t)) \right) & if $i\not\in \tilde{S}(t)$ \\
      w_i(t)        & otherwise
    \end{cases*}
\end{align*}\label{alg:update_weights_adversarial}
\STATE $t\leftarrow t+1$
\ENDWHILE{}
\end{algorithmic}
\end{algorithm}

\begin{theorem}\label{thm:adversarial_case_bound}
Algorithm \texttt{Exp3.M.B} achieves regret
\begin{align*}
\mathcal{R} \leq 2.63\sqrt{1 + \frac{B}{g c_{\min}}} \sqrt{gN\log(N/K)} + K,
\end{align*}
where $g$ is the maximal gain of the optimal algorithm. This bound is of order $O(\sqrt{BN\log(N/K)})$.
\end{theorem}
The runtime of Algorithm \texttt{Exp3.M.B} and its space complexity is linear in the number of arms, i.e. $O(N)$. See the appendix for the proof.

\subsection{Upper Bound on the Regret without $g$}
If no such bound $g$ exists, we have to modify Algorithm \ref{alg:Adversarial_Budget_Constrained}. Specifically, the weights are now updated in the following fashion:
\begin{align}
w_i(t+1) =
    \begin{cases*}
      w_i(t) \exp\left( \frac{K\gamma}{N}(\hat{r}_i(t) - \hat{c}_i(t)) \right) & if $i\in S(t)$ \\
      w_i(t)        & otherwise
    \end{cases*}
\end{align}
This replaces the original update step in line \ref{alg:update_weights_adversarial} of Algorithm \ref{alg:Adversarial_Budget_Constrained}. As in Algorithm \texttt{Exp3.1} in \cite{Auer:2002aa}, we use an adaptation of Algorithm \ref{alg:Adversarial_Budget_Constrained}, which we call \texttt{Exp3.1.M}, see Algorithm \ref{alg:Exp3.1.M}. In Algorithm \ref{alg:Exp3.1.M}, we use the following notation:
\begin{align}
\hat{G}_i(t) = \sum_{s=1}^t \hat{r}_i(s).
\end{align}

\begin{algorithm}[h!]
\caption{Algorithm \texttt{Exp3.1.M} with fixed number of plays $T$}
\label{alg:Exp3.1.M}
\textbf{Input:} $K$, Arms $1, \ldots, N$. \\
\textbf{Initialize:} $t=1$, $w_i = 1$ for $i\in [N]$, $r=0$.
\begin{algorithmic}[1]
\WHILE {$t \leq T$}
\STATE Define $g_r = \frac{N\log(N/K)}{e-1}4^r$
\STATE Restart \texttt{Exp3.M} with $\gamma_r = \min\left(1, 2^{-r} \right)$
\WHILE {$\max_{S\in\mathcal{S}} \sum_{i\in S}\hat{G}_i(t) \leq g_r - \frac{N}{K\gamma_r}$}\label{alg:termination_criterion_exp31m}
\STATE Choose random action $S(t)$ with \texttt{DependentRounding}, observe $r_i(t)$ for $i\in S(t)$, calculate $\hat{r}_i(t)$.
\STATE $\hat{G}_i(t) \to \hat{G}_i(t) + \hat{x}_i(t)$ for $i \in [N]$
\STATE $t\to t + 1$
\ENDWHILE {}
\STATE $r\to r+1$
\ENDWHILE {}
\RETURN Gain $G_{\texttt{Exp3.1.M}}$
\end{algorithmic}
\end{algorithm}

\begin{proposition}\label{prop:upper_bound_no_g_no_budget}
For the multi-play case and without budget, the regret is upper bounded by
\begin{align}\label{eq:prop_upper_bound_no_g_no_budget}
G_{\max} - \mathbb{E}[G_{\texttt{Exp3.1.M}}] \leq 8\sqrt{e-1}\sqrt{G_{\max}N\log\left(\frac{N}{K}\right)} + 8(e-1)\frac{N}{K} + 2N\log\left(\frac{N}{K}\right)
\end{align}
\end{proposition}
Note that for $K=1$ we recover Theorem 4.1 from \cite{Auer:2002aa}. To derive such a bound for the case with budget, we make the following Assumption:
\begin{assumption}\label{as:incentive_compatibility}
$\sum_{i\in S} r_i(t) \geq \sum_{i\in S} c_i(t)$ for all $S \in \mathcal{S}$ of size $K$ and $t \geq 1$.
\end{assumption}
Assumption \ref{as:incentive_compatibility} is a natural assumption, which is motivated by ``incentive compatibility'' reasons. In other words, a user will only play the bandit algorithm if the reward is greater than the cost that incurs for playing.

\begin{proposition}\label{prop:upper_bound_no_g}
For the multi-play case with budget, the regret is upper bounded by
\begin{equation}
\begin{aligned}
G_{\max} - \mathbb{E}[G_{\texttt{Exp3.1.M.B}}] &\leq 8 \sqrt{(e-1)-(e-2)c_{\min}}\sqrt{(G_{\max}-B+K)N\log(N/K)} \\
&\quad +8\left[(e-1)-(e-2)c_{\min}\right]\frac{N}{K} + 2N\log(N/K) + K
\end{aligned}
\end{equation}
\end{proposition}
This bound is derived from Algorithm \texttt{Exp3.1.M.B} (Algorithm \ref{alg:Exp3.1.M.B}), which differs from Algorithm \texttt{Exp3.1.M} (\ref{alg:Exp3.1.M}) only in the definition of $g_r$ (\ref{alg:g_r_definition_exp31mB}) and the termination criterion (line \ref{alg:termination_criterion_exp31mB}). See Algorithm \ref{alg:Exp3.1.M.B}  In Algorithm \texttt{Exp3.1.M.B}, $\hat{L}_i(t)$ denotes the sum of expected costs up to time $t$:
\begin{align}
\hat{L}_i(t) &= \sum_{s=1}^t \hat{c}_i(s).
\end{align}
Notice that if $c_{\min}=0$ and $B=0$, that is, in the case of zero per-round costs and a zero budget, which corresponds to the setting in Proposition \ref{prop:upper_bound_no_g_no_budget}, we almost recover \eqref{eq:prop_upper_bound_no_g_no_budget} with the exception of the constant $K$. This constant is due to the fact that the budget $B$ is not perfectly exhausted, because the algorithm terminates whenever the sum of current costs observed in the round of termination, $Kc_{\max} = K$, exceeds the remaining budget.

\begin{algorithm}[h!]
\caption{Algorithm \texttt{Exp3.1.M.B} with Budget $B$}
\label{alg:Exp3.1.M.B}
\textbf{Input:} $K$, Arms $1, \ldots, N$, Budget $B$. \\
\textbf{Initialize:} $t=1$, $w_i = 1$ for $i\in [N]$, $r=0$.
\begin{algorithmic}[1]
\WHILE {$\sum_{t=1}^T \sum_{i\in S(t)} c_i(t) \leq B$}
\STATE Define $g_r = \frac{N\log(N/K)}{(e-1)-(e-2)c_{\min}}4^r$ \label{alg:g_r_definition_exp31mB}
\STATE Restart \texttt{Exp3.M.B} with $\gamma_r = \min\left(1, 2^{-r} \right)$
\WHILE {$\max_{S\in\mathcal{S}} \sum_{i\in S}(\hat{G}_i(t) - \hat{L}_i(t)) \leq g_r - \frac{N(1-c_{\min})}{K\gamma_r}$}\label{alg:termination_criterion_exp31mB}
\STATE Choose random action $S(t)$ with \texttt{DependentRounding}, observe $r_i(t)$ and $c_i(t)$ for $i\in S(t)$, calculate $\hat{r}_i(t)$ and $\hat{c}_i(t)$.
\STATE $\hat{G}_i(t) \to \hat{G}_i(t) + \hat{r}_i(t)$ for $i \in [N]$
\STATE $\hat{L}_i(t) \to \hat{L}_i(t) + \hat{c}_i(t)$ for $i \in [N]$
\STATE $t\to t + 1$
\ENDWHILE {}
\ENDWHILE {}
\RETURN Gain $G_{\texttt{Exp3.1.M.B}}$
\end{algorithmic}
\end{algorithm}

\subsection{Lower Bounds on the Regret}

\begin{theorem}\label{thm:lower_bound_single_play}
For $K=1$ (single arm play), we can derive the following lower bound on the regret:
\begin{align}\label{eq:lower_bound_regret_single_play_eps}
\mathcal{R} \geq \varepsilon \left( B - \frac{B}{N} - 2Bc_{\min}^{-3/2}\varepsilon \sqrt{\frac{B\log(4/3)}{N}} \right)
%\mathcal{R} \geq \varepsilon B\left( (1-c_{\min}) - \frac{\varepsilon}{4c_{\min}^{3/2}}\sqrt{\frac{B}{N}\log(4/3)} \right),
%\mathcal{R} \geq \varepsilon\left( \frac{2B}{1+c_{\min}} - \frac{2B}{N(1+c_{\min})} - \frac{4B\varepsilon}{c_{\min}^{3/2}}\sqrt{\frac{2B\log(4/3)}{N(1+c_{\min})}} \right),
\end{align}
where $\varepsilon \in (0, 1/4)$. Choosing $\varepsilon$ as
\begin{align}
\varepsilon = \min\left(\frac{1}{4},~\frac{(1-1/N)c_{\min}^{3/2}}{4\sqrt{\log(4/3)}}\sqrt{\frac{N}{B}}\right)
%\varepsilon = \min\left(\frac{1}{4},~\frac{(1-c_{\min})c_{\min}^{3/2}}{2}\sqrt{\frac{N}{8\log(4/3) B}}\right)
%\varepsilon = \min\left(\frac{1}{4},~\frac{c_{\min}^{3/2}}{8\sqrt{2\log(4/3)}\sqrt{1+c_{\min}}} \sqrt{\frac{N}{B}}\right)
\end{align}
yields the bound
\begin{align}\label{eq:lower_bound_regret_single_play}
\mathcal{R} \geq \min\left(\frac{c_{\min}^{3/2}}{8\sqrt{\log(4/3)}}(1-1/N)^2\sqrt{NB} ,~\frac{1}{8}B(1-1/N)\right)
%\mathcal{R} \geq \min\left(\frac{(1-c_{\min})^2 c_{\min}^{3/2}}{8\sqrt{2\log(4/3)}}\sqrt{NB} ,~\frac{1}{8}B(1-c_{\min})\right)
%\mathcal{R} \geq \min\left( 0.082 \left( \frac{c_{\min}}{1+c_{\min}} \right)^{3/2}\sqrt{BN},~\frac{7}{32}\frac{B}{1+c_{\min}} \right)
\end{align}
\end{theorem}
See Appendix \ref{sec:lower_bound_single_play} for the proof.

\begin{theorem}\label{thm:lower_bound_multiple_play}
For $K>1$ (multiple play), we can derive the following lower bound on the regret:
\begin{align}\label{eq:lower_bound_regret_multiple_play_eps}
\mathcal{R} \geq \varepsilon\left( B - \frac{BK}{N} - 2Bc_{\min}^{-3/2}\varepsilon\sqrt{\frac{BK\log(4/3)}{N}} \right),
\end{align}
where $\varepsilon \in (0, 1/4)$. Choosing $\varepsilon$ as
\begin{align}
\varepsilon = \min\left(\frac{1}{4},~\frac{(1-K/N)c_{\min}^{3/2}}{4\sqrt{\log(4/3)}}\sqrt{\frac{N}{BK}}\right)
\end{align}
yields the bound
\begin{align}\label{eq:lower_bound_regret_multiple_play}
\mathcal{R} \geq \min\left(\frac{c_{\min}^{3/2}}{8\sqrt{\log(4/3)}}(1-K/N)^2\sqrt{\frac{NB}{K}} ,~\frac{1}{8}B(1-K/N)\right)
\end{align}
\end{theorem}
See Appendix \ref{sec:lower_bound_multiple_play} for the proof.

\subsection{High Probability Bounds}
For a fixed number of rounds (no budget considerations) and single play per round ($K=1$), \cite{Auer:2002aa} derived the following upper bound on the regret that holds with probability at least $1-\delta$:
\begin{align}
G_{\max} - G_{\texttt{Exp3.P}} \leq 4\sqrt{NT \log\left( NT/\delta\right)} + 4\sqrt{\frac{5}{3}NT\log N} + 8\log\left( \frac{NT}{\delta}\right)
\end{align}
\begin{theorem}\label{thm:multiple_play_fixed_round_high_probability}
For the multiple play algorithm ($1\leq K \leq N$) and a fixed number of rounds $T$, the following bound on the regret holds with probability at least $1-\delta$:
\begin{align}\label{eq:high_probability_bound_multiple_play_fixed_T}
\mathcal{R} = G_{\max} - G_{\texttt{Exp3.P.M}} &\leq 2\sqrt{5}\sqrt{NKT\log(N/K)} + 8\frac{N-K}{N-1}\log\left( \frac{NT}{\delta} \right) \nonumber\\
&\quad+ 2(1+K^2)\sqrt{NT\frac{N-K}{N-1}\log\left( \frac{NT}{\delta} \right)}
\end{align}
\end{theorem}
Theorem \ref{thm:multiple_play_fixed_round_high_probability} can be derived by using Algorithm \ref{alg:Exp3.P.M}, which is a combination between Algorithm \ref{alg:Adversarial_Budget_Constrained} and Algorithm \texttt{Exp3.P} in \cite{Auer:2002aa}. See Appendix \ref{sec:proof_Exp3PM} for the proof.

\begin{algorithm}[h]
\caption{\texttt{Exp3.P.M} for fixed number of rounds $T$}
\label{alg:Exp3.P.M}
\textbf{Input:} Number of Rounds $T > 1$, parameter $\gamma \in (0, 1]$, confidence parameter $0 < \delta < 1$\\
\textbf{Initialize:} $t=1$; $\alpha = 2\sqrt{\frac{N-K}{N-1} \log\left( \frac{NT}{\delta} \right)}$. For $i\in [N]$:
\begin{align}\label{eq:weights_exp3pm}
w_i(1) = \exp\left( \frac{\alpha \gamma K^2}{3}\sqrt{\frac{T}{N}} \right)
\end{align}
\begin{algorithmic}[1]
\FOR {$t=1, \ldots, T$}
\IF {$\arg\max_{i\in [N]} w_i(t) \geq \left(\frac{1}{K} - \frac{\gamma}{N} \right)\sum_{j=1}^N \frac{w_i(t)}{1-\gamma}$}
\STATE Determine $v_t$ as follows:
\begin{align*}
\frac{v_t}{\sum_{i=1}^N v_t \cdot\mathds{1}(w_i(t) \geq v_t) + w_i(t)\cdot\mathds{1}(w_i(t) < v_t)} = \frac{1/K - \gamma/N}{1-\gamma}
\end{align*}
\STATE Define set $\tilde{S}(t) = \lbrace i\in [N]~|~w_i(t) \geq v_t\rbrace$.
\STATE Define weights $\tilde{w}_i(t) = v_t$ for $i\in\tilde{S}(t)$.
\ELSE
\STATE Define set $\tilde{S}(t) = \lbrace\rbrace$.
\ENDIF{}
\STATE Define weights $\tilde{w}_i(t) = w_i(t)$ for $i\in [N]\setminus \tilde{S}(t)$.
\STATE Calculate probabilities:
\begin{align*}
p_i(t) = K\left( (1-\gamma)\frac{\tilde{w}_i(t)}{\sum_{j=1}^N \tilde{w}_j(t)} + \frac{\gamma}{N} \right)~\text{for } i\in\tilde{S}(t).
\end{align*}
\STATE Draw $S(t) \leftarrow$ \texttt{DependentRounding}$(K, (p_1, \ldots, p_N))$.
\STATE Pull arms $S(t)$, observe rewards $r_i(t)\in [0, 1]$.
\STATE Calculate estimated rewards and update weights for each $i\in [N]$:
\begin{align*}
\hat{r}_i(t) &=
    \begin{cases*}
      r_i(t) / p_i(t) & if $i\in S(t)$ \\
      0        & otherwise
    \end{cases*}\hspace*{1.5cm} \\
    w_i(t+1) &=
    \begin{cases*}
      w_i(t) \exp\left[ \frac{\gamma K}{3N}\left(\hat{r}_i(t) + \frac{\alpha}{p_i(t)\sqrt{NT}}\right) \right] & if $i\not\in \tilde{S}(t)$ \\
      w_i(t)        & otherwise
    \end{cases*}
\end{align*}\label{alg:update_weights_Exp3.P.M}
\ENDFOR{}
\RETURN Gain $G_{\texttt{Exp3.P.M}}$.
\end{algorithmic}
\end{algorithm}

\begin{theorem}\label{thm:multiple_play_budget_high_probability}
For the multiple play algorithm ($1\leq K \leq N$) and the budget $B > 0$, the following bound on the regret holds with probability at least $1-\delta$:
\begin{align}\label{eq:high_probability_bound_budget}
\mathcal{R} = G_{\max} - G_{\texttt{Exp3.P.M.B}} &\leq 2\sqrt{3}\sqrt{\frac{NB(1-c_{\min})}{c_{\min}}\log\frac{N}{K}} + 4\sqrt{6}\frac{N-K}{N-1}\log\left( \frac{NB}{Kc_{\min}\delta} \right) \nonumber\\
&\quad+ 2\sqrt{6}(1+K^2)\sqrt{\frac{N-K}{N-1}\frac{NB}{Kc_{\min}}\log\left( \frac{NB}{Kc_{\min}\delta} \right)}
\end{align}
\end{theorem}
To derive bound \eqref{eq:high_probability_bound_budget}, we use Algorithm \ref{alg:Exp3.1.M.B}, but with the following update rule (line \ref{alg:update_weights_Exp3.P.M} in Algorithm \ref{alg:Exp3.1.M.B}) for the weights in order to incorporate information about estimated costs:
\begin{align}\label{eq:update_weights_Exp3.P.M.B}
w_i(t+1) = \begin{cases*}
w_i(t) \exp\left[ \frac{\gamma K}{3N}\left(\hat{r}_i(t) - \hat{c}_i(t) + \frac{\alpha\sqrt{Kc_{\min}}}{p_i(t)\sqrt{NB}}\right) \right] & if $i\not\in \tilde{S}(t)$ \\
      w_i(t)        & otherwise
    \end{cases*}
\end{align}
The weights are initialized as follows:
\begin{align}
w_i(1) = \exp\left( \frac{\alpha\gamma K^2}{3}\sqrt{\frac{B}{NKc_{\min}}} \right)
\end{align}
In addition, the estimated costs $\hat{c}_i(t)$ are computed as $\hat{c}_i(t) = c_i(t)/p_i(t)$ whenever arm $i$ is pulled at time $t$. 

==> Sections/StochasticCase.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% This is StochasticCase.tex (part of BudgetConstrainedMAB.tex)
% author: Datong Zhou
% last edited: August 17, 2017
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% !TEX root = ../BudgetConstrainedMAB.tex
\section{Stochastic Case}

\subsection{Problem Formulation}
The player is given a budget $0 < B \in\mathbb{R}_+$ to pull arms of a multi-armed bandit. Each arm $i\in [N]$ is endowed with an unknown reward and cost distribution with means $0 < \mu_r^i \leq 1$ and $0 < c_{\min} \leq \mu_c^i \leq 1$, respectively. At each time step, exactly $K$, $1 \leq K \leq N$ arms have to be pulled. For each arm $i\in a_t$ pulled at time $t$, a cost $c_{i,t}\in [c_{\min}, 1]$ and reward $r_{i,t}\in [0, 1]$ are generated according to the underlying reward and cost distribution, independently of previous costs and rewards. In this paper, we analyze the \textit{semi-bandit} setting, in which the player observes the realizations of $c_{i,t}$ and $r_{i,t}$ for each arm $i\in a_t$. The player does not observe the rewards or costs for arms not pulled. At the end of each round, the user pays for the realized costs $\sum_{i\in a_t}c_{i,t}$ with its current budget and obtains payoff $\sum_{i\in a_t}r_{i,t}$, unless the current round cost exceeds the remaining budget, in which case the game terminates.

Notice the minimum threshold $c_{\min}$ on the support of the cost distributions. This assumption is not just of a practical nature, since many applications of bandits come with a minimum cost, but also due to the necessity of well-defined ``bang-per-buck'' ratios $\mu_r^i / \mu_c^i$, which our analyses throughout this paper heavily rely on.

In this section, we design a deterministic algorithm $\mathcal{A}$ such that the expected payout is maximized, given the budget constraint and the constraint that exactly $K$ arms have to be pulled. Formally:
\begin{equation}\label{eq:bandit_optimization}
\begin{aligned}
& \underset{a_1, \ldots, a_{\tau_{\mathcal{A}}(B)}}{\text{maximize}}
& & \mathbb{E}\left[ \sum_{t=1}^{\tau_{\mathcal{A}}(B)} \sum_{i\in a_t} r_{i,t} \right] \\
& \text{subject to}
& & \mathbb{E}\left[ \sum_{t=1}^{\tau_{\mathcal{A}}(B)} \sum_{i\in a_t} c_{i,t} \leq B \right] \\
& & & a_t \in \lbrace 0, 1\rbrace^N, \quad \mathbf{1}\cdot a_t = K~\forall~t\in [\tau_{\mathcal{A}}(B)]
\end{aligned}
\end{equation}
In \eqref{eq:bandit_optimization}, $\tau_{\mathcal{A}}(B)$ is the stopping time of algorithm $\mathcal{A}$ and indicates after how many steps the algorithm terminates, namely when the budget is exhausted. $a_t$ is a binary vector consisting of exactly $K$ ones and $N-K$ zeros. The expectation is taken over the randomness of the reward and cost distributions.

\subsection{Definitions}
Let $n_{i,t}$ denote the number of times arm $i$ has been played until time $t$. Let $\bar{\mu}_{r}^{n_{i,t}}$ and $\bar{\mu}_{c}^{n_{i,t}}$ denote the empirical mean of rewards and costs observed for arm $i$ up to time $t$, respectively. Let $\bar{\mu}^{n_{i,t}}$ denote their ratio, that is,
\begin{align}\label{eq:empirical_bang_per_buck_ratio}
\bar{\mu}^{n_{i,t}} = \frac{\bar{\mu}_{r}^{n_{i,t}}}{\bar{\mu}_{c}^{n_{i,t}}}.
\end{align}
Further, let $\mu_i := \mu_r^i / \mu_c^i$ denote the ground truth ratio of mean reward to mean cost of arm $i$. 

At each round, the $K$ arms with the highest upper confidence bounds are pulled. The upper confidence bound $U_{i,n_{i,t}}$ of arm $i$ consists of the empirical mean of all $n_{i,t}$ observed bang-per-buck ratios obtained for arm $i$ until time $t$, namely \eqref{eq:empirical_bang_per_buck_ratio}, and an exploration term $e_{n_{i,t}}$:
\begin{align}\label{eq:upper_confidence_bound}
U_{n_{i,t}} = \bar{\mu}^{n_{i,t}} + e_{n_{i,t}}
\end{align}
For the sake of notational ease, we write $U_{n_{i,t}} = U_{i,t}$, $\bar{\mu}^{n_{i,t}} = \bar{\mu}_t^i$, $e_{n_{i,t}} = e_{i,t}$, $\bar{\mu}_r^{n_{i,t}} = \bar{\mu}_{r,t}^i$, and $\bar{\mu}_c^{n_{i,t}} = \bar{\mu}_{c,t}^i$, hence dropping the explicit $n_{i,t}$ notation whenever it is clear from context, while keeping in mind that the number of times arm $i$ has been played until round $t$ affects these variables. The exploration term $e_{i,t}$ will be defined at a later point.

Let $a^\ast$ denote the selection of the $K$ optimal arms with the $K$ highest bang-per-buck ratios. Morever, let $\Delta_{a_t}$ denote the difference between the sum of expected bang-per-buck ratios for choice $a_t$ and the optimal choice $a^\ast$:
\begin{align}\label{eq:Delta_a_definition}
\Delta_{a_t} := \sum_{i\in a^\ast}\frac{\mu_r^i}{\mu_c^i} - \sum_{i\in a_t} \frac{\mu_r^i}{\mu_c^i}
\end{align}
We write $\Delta_{\max}$ for the choice of $a_t$ that maximizes the quantity $\Delta_{a_t}$, that is, $\Delta_{\max} = \max_{a_t}\Delta_{a_t}$. Lastly, let $\rho_{a_t}$ denote the differences in expected per-round payouts between $a_t$ and $a^\ast$:
\begin{align}\label{eq:rho_at_definition}
\rho_{a_t} := \sum_{i\in a^\ast} \mu_r^i - \sum_{i\in a_t}\mu_r^i.
\end{align}
As in \eqref{eq:Delta_a_definition}, $\rho_{\max} = \max_{a_t}\rho_{a_t}$. 


\subsection{Algorithm}
Algorithm \ref{alg:Comb_MAB_Budget_Constrained} describes the algorithm $\mathcal{A}$ to pull exactly $K$ arms at each round until the budget is exhausted. For initialization purposes, all $N$ arms are played exactly once prior to the while-loop. In each subsequent round, the $K$ arms with the highest upper confidence bounds $U_{i,t}$ (line \ref{alg:UCB}) are played and the rewards as well as the costs are observed. The algorithm terminates when the cost of the currently pulled arms exceeds the remaining budget.

\begin{algorithm}[h]
\caption{Budget Constrained Combinatorial Multi-Armed Bandit}
\label{alg:Comb_MAB_Budget_Constrained}
\textbf{Input:} Budget $B > 0$, arms $1, \ldots, N$ with mean rewards $\mu_r^i$ and costs $\mu_c^i$, and $K$. \\
\textbf{Initialize:} $t=1$. Pull all arms together once. Let $\bar{\mu}_{r,1}^i = r_{i,1}$, $\bar{\mu}_{c,1}^i = c_{i,1}$, $\bar{\mu}_1^i = \frac{\bar{\mu}_{r,1}^i}{\bar{\mu}_{c,1}^i}~\forall~i\in [N]$, $n_{i,1} = 1$, $e_{i,1} = \texttt{Double.MAX\textunderscore VALUE}~\forall~i\in [N]$. $U_{\mathcal{A}} = 0$.

\begin{algorithmic}[1]
\WHILE {$B > 0$}
\STATE $a_t \gets$ Pull $K$ arms associated with $K$ largest $U_{i,t}$. \label{alg:UCB}
\IF {$\sum_{j\in a_t} c_{j,t} > B$}
\RETURN Payout $U_{\mathcal{A}}$, stopping time $\tau_{\mathcal{A}}(B) = t$ \label{alg:return}
\ENDIF{}
\STATE Update payout and remaining budget: $U_{\mathcal{A}} \gets U_{\mathcal{A}} + \sum_{i\in a_t}r_{i,t}$, $\quad B \gets B - \sum_{i\in a_t} c_{i,t}$
%\STATE Update empirical bang-per-buck ratios
\STATE $t\gets t+1$
\STATE $e_{i,t} \gets \begin{cases*}
      \frac{\sqrt{(K+1)\log t / n_{i,t}}(1+1/c_{\min})}{c_{\min} - \sqrt{(K+1)\log t / n_{i,t}}} & if $c_{\min} > \sqrt{(K+1)\log t / n_{i,t}}$ \\
      \texttt{Double.MAX\textunderscore VALUE}        & otherwise
    \end{cases*} ~\forall~i\in [N]$ \label{alg:UCB_update}
\ENDWHILE{}
\end{algorithmic}
\end{algorithm}

Notice that the denominator of the exploration term $e_{i,t}$ can become negative, in which case we assign a large positive number to $e_{i,t}$. The $O(\log B)$ upper bound on the regret is not impacted by this operation, because after a sufficient number of plays, we have $n_{i,t} \gg (K+1)\log t$.

\subsection{Analysis of the Algorithm}
In this section, we show that Algorithm \ref{alg:Comb_MAB_Budget_Constrained} achieves logarithmic regret in the budget $B$, where we define the regret to be the difference between the expected payout under the optimal strategy (which has access to all bang-per-buck ratios), $\mathbb{E}[U_{\mathcal{A}^\ast}]$, and the expected payout under algorithm \ref{alg:Comb_MAB_Budget_Constrained}, $\mathbb{E}[U_{\mathcal{A}}]$:
\begin{align}\label{eq:regret_definition}
\mathcal{R}(B) = \mathbb{E}[U_{\mathcal{A}^\ast}(B)] - \mathbb{E}[U_{\mathcal{A}}(B)]
\end{align}
In \eqref{eq:regret_definition}, the expectation is taken with respect to the distribution of rewards and costs. The algorithm itself is deterministic.

\begin{theorem}\label{thm:stochastic_case_sublinear_regret}
Algorithm \ref{alg:Comb_MAB_Budget_Constrained} achieves regret $\mathcal{R}(B) = O(NK^4 \log B)$.
\end{theorem}
The prove Theorem \ref{thm:stochastic_case_sublinear_regret}, we bound the number of suboptimal choices made by the algorithm (Section \ref{sec:stochastic_bound_num_subopt_choices}). In addition, we approximate the stopping time of the algorithm (Section \ref{sec:stochastic_bound_stopping_time}). Both components allow for the derivation of an upper bound on the regret (Section \ref{sec:stochastic_bound_regret}).

